DONeRF: Towards Real-Time Rendering of Compact Neural Radiance Fields using Depth Oracle Networks

The recent research explosion around implicit neural representations, such as NeRF, shows that there is immense potential for implicitly storing high-quality scene and lighting information in compact neural networks. However, one major limitation preventing the use of NeRF in real-time rendering applications is the prohibitive computational cost of excessive network evaluations along each view ray, requiring dozens of petaFLOPS. In this work, we bring compact neural representations closer to practical rendering of synthetic content in real-time applications, such as games and virtual reality. We show that the number of samples required for each view ray can be significantly reduced when samples are placed around surfaces in the scene without compromising image quality. To this end, we propose a depth oracle network that predicts ray sample locations for each view ray with a single network evaluation. We show that using a classification network around logarithmically discretized and spherically warped depth values is essential to encode surface locations rather than directly estimating depth. The combination of these techniques leads to DONeRF, our compact dual network design with a depth oracle network as its first step and a locally sampled shading network for ray accumulation. With DONeRF, we reduce the inference costs by up to 48x compared to NeRF when conditioning on available ground truth depth information. Compared to concurrent acceleration methods for raymarching-based neural representations, DONeRF does not require additional memory for explicit caching or acceleration structures, and can render interactively (20 frames per second) on a single GPU.

==> method_old.tex <==
\section{Efficient Neural Rendering}
\label{sec:method}

To seamlessly support large scenes, we split the scene into slightly overlapping view cells. 
Every cell corresponds to a 3D position and an angle range describing the possible camera rotations and thus a 5D slice of potential viewing rays in the scene.
For our setup, we typically use view cells of \SI[parse-numbers=false]{2\times2\times2}{\meter}\todo{is this correct yet?} and viewing rays spanning \SI{270}{\degree}.
For every view cell, we generate one \gls{nsr} that is then used to generate novel views within this cell.
If the user moves out of one view cell, either by translation or rotation, rendering continues from the next view cell.
In this paper, we only consider static geometry and lighting, focusing on the possibility to efficiently render \glspl{nsr}.


For \gls{nsr} generation, \ie, training, we use RGBD input images sampled from the view cell.
In comparison to the original \gls{nerf} work, we require additional depth information, which is available for generated content. 
For captured content, we can first construct a densely sampled \gls{nerf} or use other depth estimation techniques to provide a sufficient depth estimate.
As we do not rely on highly accurate depth---although higher quality depth increases the potential gains for both quality and evaluation efficiency---a rough depth estimate serves as a good starting point.

\begin{figure*}[t]
	\centering
	\includegraphics[width=.7\linewidth]{figures/pipeline}
	\caption{\todo[inline]{Approach overview}To enable efficient rendering of large scenes with neural radiance fields, we propose a five stage pipeline: (1) ray descriptions are unified within a view cell, (2) depth is considered in a non-linear space, (3) an oracle network estimates the importance of sample locations along each view ray, (4) those sample locations are warped spherically towards the view cell, and (5) radiance information is generated using another \gls{mlp} sampling only few locations along each ray.}
	\label{fig:overview}
\end{figure*}

Our approach consists of two networks, whereas the second follows a standard \gls{nerf}-style setup:
An \gls{mlp} which evaluates multiple sample points along a ray with volume integration via its RGBA output.
The network is fed with Fourier-encoded~\cite{tancik2020fourfeat} 3D sample positions and the corresponding view ray direction, with the encoded direction being added to the last layer of the network.
However, we replace the coarse network of the original \gls{nerf} work with a depth oracle network and propose different transformations on the data at various points throughout the network chain to support more efficient rendering.

Our network chain is shown in Figure~\ref{fig:overview}:
At first, we transform the input rays to a unified space, given information about the supported view cell (\emph{Ray Unification}, Section \ref{sec:SphPosDir}).
Second, we use a depth oracle network to predict good sample locations along the view ray (\emph{Oracle Network}, Section \ref{sec:DepthLayers}).
Third, we place a low amount of samples in the vicinity of the estimated depth, allowing us to efficiently sample in the local region of interest (\emph{Local NeRF}, Section \ref{sec:localsampling}).
For large scenes, we transform both the depth and local samples non-linearly (\emph{Non-Linear Depth}, Section \ref{sec:NLDepthSpaceWarping}), and use additional spherical space warping for sampling the Local NeRF (\emph{Space Warping}, Section \ref{sec:NLDepthSpaceWarping}).

\subsection{Local Sampling}
\label{sec:localsampling}
One of the major hurdles in using \glspl{nerf} for efficient rendering is the shear cost of evaluating the network hundreds of times along each view ray.
One straightforward idea to enable efficient rendering is to reduce the number of ray samples.
As \gls{nerf} style volume rendering is able to produce depth maps by simply observing the optical density values output by the network, only few samples contribute to the final image, those around object surfaces---when ignoring participating media and transparencies.\todo{maybe we want to show this by plotting statistics for full nerfs and showing that empty space mostly does not contribute? would be an interesting early plot}

To this end, placing samples where they contribute most to the final image will increase rendering performance.
A first approach to provide such sample locations was already investigated in the original \gls{nerf} in the form of the coarse-fine network architecture.
Not relying on a network, but rather using an additional data structure, one can use an octree to bound \gls{nerf} sampling \todo{cite}.
However, an octree requires an additional data structure, it must be traversed for each ray and the scaling to large scenes becomes questionable.

In any case, relying on localized sampling guided by an oracle has multiple advantages:
First, \gls{nerf} evaluation can be sped up significantly, as few samples are sufficient to generate high quality images, see Figure \ref{fig:teaser}.
Second, supervised learning for localized samples reduces training time significantly, as the network does not need to learn about empty space.\todo{if we state this claim here, we need to also provide data / results for it, i.e., how much the training time differs}
Third, the network can spend its capacity on the important samples that contribute to the final image and does not need to learn the optical density for empty space. 
Thus, the overall image quality is increased compared to a network that is also sampled in empty space (Figure \ref{fig:teaser} upper row).

Obviously, local sampling comes with downsides.
First, handling transparencies is more difficult. 
One needs to place samples not only at opaque surfaces but also where transparent objects are hit.\todo{we could also ignore transparent objects and view them as view-dependent effects on the surfaces behind them?}
Second, providing correct local sample locations requires a capable oracle.

\subsection{Oracle Network}
\label{sec:DepthLayers}
In our work, we use another \gls{mlp} as an oracle to predict ideal local sampling locations.
The oracle network takes a ray description as input and provides information about where samples should be placed along that ray.
While providing depth estimates for a view cell initially sounds not overly difficult, it is non-trivial if those depth estimates must be as close as possible to the surface locations, especially around depth discontinuities.
Using an \gls{mlp} of the same size as we use for the \gls{nerf} produces sufficiently accurate estimates for the majority of rays in simple scenes.
However, even for simple scenes, accurate estimates around depth discontinuities are difficult to predict, as shown in Figure \ref{fig:depthoutline}.


\begin{figure}
	\centering
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/single_depth_0}
		\caption{Depth Prediction}
	\end{subfigure}%
	\hfill%
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/single_depth_1}
		\caption{Local Raymarching}
	\end{subfigure}
	\caption{\todo[inline]{remake figure with fewer samples - direct depth prediction blurres depth at discontinuities and thus surfaces are missed - see white outline - make zoom in}}
	\label{fig:depthoutline}
\end{figure}


To mitigate this issue, we make the following observation: in general, the exact geometric structure of the scene is faithfully reconstructed using \gls{nerf} style rendering, where samples are also placed in empty space.
Thus, we can provide the oracle network more freedom; while it must at least provide a depth estimate on the hit surface, it can also provide \emph{additional} estimates. 
In case of depth discontinuities, the foreground edge and the object right behind could be returned by the oracle.
Thus, the overall rendering result will be correct, even if two neighboring rays, one hitting the foreground object and one a background object, are both sampled at the foreground and the background, see Figure \ref{fig:multidepth_target_sampling}
In case multiple edges are stacked in depth, the oracle can provide depth estimates for all layers.

\begin{figure}
	\centering
	\includegraphics[page=4,width=0.7\linewidth]{figures/depth_sheets}
	\caption{\todo[inline]{drawing for multidepth output}Visualization of a ray slice cutting through the bulldozer model at about two thirds of the height. The oracle can produce multiple depth outputs, as long as one sample lands on the surface, the other one can be freely placed an the correct color can still be reconstruct.}
	\label{fig:multidepth_target_sampling}
\end{figure}


\paragraph{Depth Sheets}
Instead of predicting a single depth estimate, we can use multiple real valued depth values as output for the oracle network, fulling our previous target description\todo{what target description? not sure what is meant here}.
The goal of the network is the following:
\begin{itemize}
	\item In case there is a single surface, one of the depth values must match the target depth as closely as possible. The other depth values can be arbitrary.
	\item For any edge (depth discontinuity) near the ray, both the foreground and background depth values of each edge should be represented in the outputs.
\end{itemize}
\todo[inline]{obviously this could be extended to transparencies}

Given a potentially variable amount of depth discontinuities that might not match the number of network outputs, it is questionable what the target of the other outputs should be in case there is only a single visible surface.
As \gls{nerf} is perfectly capable of learning empty space, we do not need to restrict the network to collapse out outputs to the surface depth and rather can provide the network more freedom.
During inference, the system is not able to distinguish whether the depth values correspond to multiple nearby depth discontinuities or whether a single surface is hit with other depth values to ignore.
Thus, samples must be placed around all oracle outputs and the \gls{nerf} network should report empty space for samples in front of the first opaque surface.
Note that the \gls{nerf} output for samples behind the first surface do not need to be punished either as they will not significantly influence the ray marching results\todo{do we need an experiment/plot/data for these things?}.
Obviously, the \gls{nerf} network must be trained for a specific oracle to learn about empty space for which the oracle demands sampling.
In the same way, it also needs to learn information around depth discontinuities. 
However, in general the \gls{nerf} networks can be very similar\todo{do you mean the weights of the networks? because the architectures can be identical and it's a bit misleading, not sure what you're referring to here} for different oracles as most samples will be placed similarly.


While the target of accurately estimating depth discontinuities is easy to specify abstractly, providing targets for supervised learning is another question.
One way to give the network the most freedom in learning \enquote{depth sheets} that wind through space is to only provide a single depth target for every training sample, \ie, the hit surface.
As the network has multiple outputs, we use a custom error metric which maps the ground truth target to the closest network output and only computes a loss (in our case MSE) against this output.
While such a setup theoretically allows the network to learn arbitrary additional depth values, learning high frequencies is typically difficult for \gls{mlp} networks, which are compactly sized---which we target for efficient evaluation anyway.
Thus, the network tends to learn smooth functions when moving in the ray space, which results in sheet-like depth estimates as seen in Figure \ref{fig:depthsheets}.


\begin{figure}
	\centering
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/depthsheets_0}
		\caption{Depth Sheets}
	\end{subfigure}%
	\hfill%
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/depthsheets_1}
		\caption{Local Raymarching}
	\end{subfigure}
	\begin{subfigure}[t]{\linewidth}
	\centering
	\includegraphics[page=3,width=0.7\linewidth]{figures/depth_sheets}
	\caption{Schematic of potential depth sheets}
	\end{subfigure}
	\caption{\todo[inline]{depth sheets color coded: every sheet in one color channel, value = depth => ther should be no hard boundaries to be seen in the depth - replace with new data}}
	\label{fig:depthsheets}
\end{figure}


However, we found that it also makes sense to supervise the network to learn multiple depth values.
To supervise the depth sheets network, we use a simple image space filter when generating target values.
We scan the surrounding of the target image pixels for a depth discontinuity above an epsilon $\epsilon_d$ in a spiral manner.
If we find such a value, we use it as an additional target and continue the spiral search until we find as many depth values that are at least $\epsilon_d$ apart, as there are outputs (or until we exceed the search window).
For $\epsilon_d$ we use the sampling distance used in the \gls{nerf} network---if distances between depth values are smaller than that, they will be sampled anyway.
Note that this filter is not the same as analyzing the scene beforehand and creating explicit depth layers by depth peeling.
While this would be possible for generated content, it may also create depth layers that will never be visible and thus waste network capacity.
Relying on the depth values from surrounding pixels/rays will only provide targets that are also visible.
As a loss function, we again use a loss that matches the estimates to the closest targets, whereas the number of targets may vary between rays.\todo{equation? don't know if it's necessary, but it's an important detail}

Also note that the more depth outputs the oracle produces, the more samples are necessary to produce an image. Typically \numrange{2}{3} samples per estimate are sufficient.
For our test scenes, we did not observe increased quality when using more than two depth estimates. \todo{do we need experiments/data/plots for that?}



\paragraph{Classified Depth}
While depth sheets achieve good results, if the number of depth layers is low, complex depth relationships become increasingly complicated to learn, especially if the number of required sheets becomes large\todo{depth layers vs. depth sheets is confusing to read - what is what?}.
Following the idea behind \gls{nerf}'s coarse network, we would like to have the oracle output sample likelihoods along the ray---\ie, a likelihood that a sample at a certain location will increase image quality.
However, we want to avoid evaluating the oracle network multiple times to keep the number of evaluations per ray low.
To this end, we increase the number of outputs of the oracle network by discretizing the space along the ray.
For every ray segment, we want a high value if it should receive (multiple) samples, a low value indicates that the segment can be skipped, see Figure~\ref{fig:classified_depth_drawing}.


\begin{figure}
	\centering
	\includegraphics[page=5,width=0.7\linewidth]{figures/depth_sheets}
	\caption{\todo[inline]{drawing for classified depth outputs}Classification output along each ray; a dark value corresponds to a high surface probability, bright values to little probability. Samples are placed accordingly, and can be used for local sampling.}
	\label{fig:classified_depth_drawing}
\end{figure}


\begin{figure*}[t]
	\begin{subfigure}[t]{.195\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal.png}
		\caption{CD-1}
	\end{subfigure}
	\begin{subfigure}[t]{.195\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{CD-5}
	\end{subfigure}
	\begin{subfigure}[t]{.195\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{CD-15}
	\end{subfigure}
	\begin{subfigure}[t]{.195\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{CD-5-5}
	\end{subfigure}
	\begin{subfigure}[t]{.195\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{CD-15-15}
	\end{subfigure}
	\caption{\todo[inline]{Examples of classified depth outputs for different filters (maybe also show predicted depth from nerf-> always the same?}}
	\label{fig:classified_depth_examples}
\end{figure*}

This turns the network into a classification network.
In the simplest setup, we discretize the depth of the surface hit by the ray as the target and use a one-hot encoding.
To train a classification network, we use the common binary cross-entropy (BCE) loss \todo{cite thomas: not sure if there is a reference for that besides a book or something}.
Typically, the network will smear out the classification results and thus will also yield non-zero outputs for rays that are close to depth discontinuities.
However, we can also use a multi-class target, enabling us to manually smear over depth values from neighboring pixels, similarly to our depth sheets filter.
For filtering we use a radial (Euclidean distance) filter to reduce the target (confidence) value of neighboring rays:
\[
xxx
\]
For example, using a $5\times5$ filter, rays being 3 pixel away contribute $0$, 2 pixels distance results in a value of $1/3$ and 1 pixel $2/3$.\todo{do we need data/experiments/plots for the filter sizes?}

From a classification point of view, filtering increases the number of false positives compared to the target surface depth, but in our case it decreases the number of false negatives overall by ensuring that we do not miss important regions of interest around the surface depth.
This becomes apparent when considering that rays exist in a continuous space, \ie, the network does not need to learn hard boundaries between rays at depth discontinuities.
Translating a higher false positive rate to ray marching, we increase the likelihoods for regions that do not need any samples.
Thus, overall, we also need to place more samples along rays to hit the \enquote{right} sample location.
However, at the same time, we reduce the chance to miss surfaces.
Given that the oracle network needs to be able to provide similar functionality as the coarse network in the original \gls{nerf} with the same capacity, but being evaluated only once instead of $100+$ times, allowing the network to move towards wrong positive classifications is essential.
Additionally, false positives can be handled by the local sampling network, as empty space will result in no image contribution.
A missed surface on the other hand would clearly reduce image quality.


Following the idea of label smoothing, we also support filtering along the labels in the depth direction, using a simple 1D Gaussian filter.
This essentially increases the positively classified cells further, enabling the oracle network to more conservatively learn the depth of surfaces.
For simple scenes, we observed that no filtering is necessary.
However, for scenes with fine structures and large view cells, both smoothing steps are essential to reduce the number of missed surfaces.
In this way, the filtering comprises a trade off between efficiency and accuracy/image quality.
See Figure \ref{fig:classified_depth_examples} for the depth oracle output for different filtering techniques.



Finally, to translate the classification values to sample locations, we use the same approach as the original \gls{nerf} when going from the coarse to the fine network:
We treat the classification output as a piecewise-constant PDF and create the sample locations using the inverse transform:
\[
xxx
\]


 

\begin{figure}
	\centering
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{}
	\end{subfigure}%
	\hfill%
	\begin{subfigure}[t]{.48\linewidth}
		\includegraphics[width=\linewidth]{figures/placeholder-normal}
		\caption{}
		\label{fig:ray_unification:disallowed}
	\end{subfigure}
	\caption{\todo[inline]{drawings for sphere pos dir with depth reduction + not allowed views for object in viewcell - b}}
	\label{fig:ray_unification}
\end{figure}
 
\subsection{Ray Unification and Oracle Input}
\label{sec:SphPosDir}
Asking the oracle network to output depth targets for all elements of the five dimensional view-cell requires the network to not only learn the surface depth, but also to solve the ambiguity of how rays can be encoded:
Rays of different camera locations may coincide, but are encoded by different ray starting positions, \eg, when moving the camera forward the center ray direction does not change, but its starting position does.
To take the burden of this computation from the network, we map every ray starting location onto a sphere circumscribed around the view cell.
To handle objects that potentially penetrate the view cell, we compute the smallest (potentially negative) depth value from the training set and use this value (minus an epsilon) as starting point for the discretization, see Figure \ref{fig:ray_unification}.
In this way, objects in the view cell reduce the possible range of camera positions by the volume of their projection to the circumscribed sphere.
In other words: the training data is not allowed to contain two images that have different depth values for the same encoding view ray, see Figure \ref{fig:ray_unification:disallowed}.


Using the unified ray position and direction as input to the oracle network, it seems intuitive to also use positional or Fourier encoding to allow the network to learn higher frequencies.
Interestingly, this did not achieve better results in our experiments.
We believe this may be due to the fact that the network needs to learn to follow the ray and compute a depth value from that single input.
A non-linear higher dimensional version of the position and direction may help little when the ray itself is a linear construct.
In contrast, during \gls{nerf} raymarching the 3D position (and directions) are used, for which repetitive patterns in typical scenes are common.

Following the intuition of asking the network to provide multiple (discretized) outputs along the ray, we additionally supply the network with as many 3D locations regularly sampled along the ray as input---the centers of the discretized depth ranges for classified depth.
Intuitively, this means that we take the coarse \gls{nerf} network and instead of querying it for each sample point, we provide all sample points as a single input and ask for as many outputs without increasing the network size.\todo{do we need experiments/data/plots for that to show that this helps?}
We again experimented with higher dimensional encoding for the input parameters, but did not reliably increase output quality.
This may be due to shear number of input parameters, which makes it more difficult for the network to learn which inputs to use.


\subsection{Non-linear Depth and Space Warping}
\label{sec:NLDepthSpaceWarping}

Large scenes (with large depth ranges) are especially difficult to handle with \gls{nerf}-style ray-casting as they require huge amounts of samples.\todo{fig? maybe refer to teaser or make another fig}
Additionally, as the view becomes deeper the empty space also increases, forcing the network to either learn mostly empty space samples and thus most spend network capacity on empty space, or to wrongly misinterpret the scene depth and fail to learn correct depth parallax for near and far objects.
While local sampling---to some degree---mitigates this issue, correctly estimating the depth also becomes more difficult, especially when using discretized depth.
As a remedy, we propose to use a non-linear quantization, enlarging the depth ranges towards the back, similarly to z-buffering in real-time rendering.
Our experiments showed that a logarithmic depth seems to work very well
$$
...
$$
This is also intuitive, as parallax and visible detail decreases towards the back, thus sample location errors in world space units are less of an issue compared to the foreground.

While a non-linear depth classification yields more fine granular depth steps in the front and increases depth steps in the back, local sampling could still use a linear space, placing samples at equal distances in world space.
Obviously, we would need to place a larger number of samples in the back to cover objects spanning the respectively larger depth steps in the back. 
Going hand in hand with the depth classification, we use the same function to space out samples along the ray, sampling elements closer to the camera with smaller steps and elements further away with larger steps.

Given that the camera can move back and forth, traditional \gls{nerf} may have a harder time with sampling, as the sampling steps in space may vary in world space, simply based on the camera location and thus sample offsets in the back may become significant.
Our ray unification mitigates this issue, as the sample distances are always relative to the sphere and not the camera position.


While non-linear depth enables us to capture the depth in larger scenes and supports adaptive local sampling, choosing the frequencies for positional and Fourier encoding is increasingly difficult according to our experiments.\todo{if we mention experiments we probably need to provide data/plots too, probably in the appendix?}
The foreground typically requires high frequencies, whereas the background details are averaged by a real camera or by mipmapping and anti-aliasing techniques for generated content.
Thus, the network needs to be provided with a large number of varying frequencies and needs to learn to selectively apply those for the foreground and background.
While we were successful to learn scenes in this manner, training takes long and typically either foreground details are missing or additional noise appears in the background.
In some cases the network is not even able to faithfully reconstruct the scene depth at all, see Figure \ref{fig:teaser}.

To remedy this issue, we propose a warping of the 3D space to work in a viewcell-centric space.
Starting from the center of the supported view cell, we warp the entire space using a radial distortion, essentially bringing the background closer to the view cell:
\[
\tilde{x} =  (x - c) \cdot W(x - c) 
\]


\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figures/placeholder-wide}
	\caption{\todo[inline]{space distortion drawing - once normal and once distorted and sample locations from two rays in both spaces}}
	\label{fig:space_distortion}
\end{figure}

We use this transformation on every single \gls{nerf} sample, \ie, we place samples in world space and then transform them before feature encoding.
While this transformation essentially warps ray samples as to not follow a straight line, all sample locations in space stay consistent, \ie, samples from different view points landing at the same 3D location are evaluated equally (ignoring the direction information), see Figure \ref{fig:space_distortion}.

According to our experiments, logarithmic warping works well, but using the inverse square root depth showed the best results:
\[
 W(p) = \frac{1}{\sqrt{|p|\cdot d_{max}}},
\]
where $d_{max}$ corresponds to the maximum scene depth and is used to normalize the location to $\pm1$ before Fourier encoding.


